Re-basin via implicit Sinkhorn differentiation

The recent emergence of new algorithms for permuting models into functionally equivalent regions of the solution space has shed some light on the complexity of error surfaces, and some promising properties like mode connectivity. However, finding the right permutation is challenging, and current optimization techniques are not differentiable, which makes it difficult to integrate into a gradient-based optimization, and often leads to sub-optimal solutions. In this paper, we propose a Sinkhorn re-basin network with the ability to obtain the transportation plan that better suits a given objective. Unlike the current state-of-art, our method is differentiable and, therefore, easy to adapt to any task within the deep learning domain. Furthermore, we show the advantage of our re-basin method by proposing a new cost function that allows performing incremental learning by exploiting the linear mode connectivity property. The benefit of our method is compared against similar approaches from the literature, under several conditions for both optimal transport finding and linear mode connectivity. The effectiveness of our continual learning method based on re-basin is also shown for several common benchmark datasets, providing experimental results that are competitive with state-of-art results from the literature.

==> Re-basin via Sinkhorn operator/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[t!]
  \centering
  \begin{tabular}{c}
    \begin{subfigure}{0.65\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/rebasin_example.pdf}
      \put(-133,35){$\theta_A$}
      \put(-125,100){$\theta_B$}
      \put(-72,35){$\pi_\mathcal{P}(\theta_B)$}
      %\caption{Loss landscape for the polynomial approximation task \cite{oswald2020continual}.}
      \caption{ }
      \label{fig:rebasin-a}
    \end{subfigure} \\
    \hspace{-10mm}
    \begin{subfigure}{0.65\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/graph.pdf}
      \put(-22,105){\tiny Naive}
      \put(-22,100){\tiny Sinkhorn}
      \put(-80,-10){$\lambda$}
      \put(-170,60){\rotatebox[origin=c]{90}{$\cost(\theta)$}}
      %\caption{Cost value within the naive linear path and after re-basin.}
      \caption{ }
      \label{fig:rebasin-b}
    \end{subfigure}
  \end{tabular}
  \caption{(a) The loss landscape for the polynomial approximation task \cite{oswald2020continual}. $\theta_A$ and $\theta_B$ are solutions found by SGD. LMC suggests that permuting hidden units of $\theta_B$ would result in $\pi_\mathcal{P}(\theta_B)$ which is functionally equivalent to before permutation, with no barrier on its linear interpolation with $\theta_A$. (b) Comparison of the cost value in the linear path before (naive) and after re-basin. The dashed line in both figures corresponds with the original (naive) path between models, and the solid line represents the path and corresponding loss after the proposed Sinkhorn re-basin.}
  \label{fig:rebasin}
\end{figure}

Despite the success of deep learning (DL) across many application domains, the loss surfaces of neural networks (NNs) are not well understood. Even for shallow neural networks, the number of saddle points and local optima can increase exponentially with the number of parameters \cite{auer1995exponentially, garipov2018loss}. The permutation symmetry of neurons in each layer allows the same function to be represented with many different parameter values of the same network. Symmetries imposed by these invariances help us to better understand the structure of the loss landscape \cite{garipov2018loss, entezari2022the, brea2019weight}.

Previous studies establish that minima found by Stochastic Gradient Descent (SGD) are not only connected in the network parameter's space by a path of non-increasing loss, but also permutation symmetries may allow us to linearly connect those points with no detriment to the loss \cite{entezari2022the, garipov2018loss, draxler2018essentially, kuditipudi2019explaining, frankle2020linear, nagarajan2019uniform}. This phenomenon is often referred to as linear mode connectivity (LMC) \cite{nagarajan2019uniform}. For instance, \cref{fig:rebasin-a} shows a portion of the loss landscape for the polynomial approximation task \cite{oswald2020continual} using the method proposed by Li \etal \cite{visualloss}. $\theta_A$ and $\theta_B$ are two minima found by SGD in different basins with an energy barrier between the pair. LMC suggests that if one considers permutation invariance, we can teleport solutions into a single basin where there is almost no loss barrier between different solutions \cite{entezari2022the, ainsworth2022git}. In literature, this mechanism is called re-basin \cite{ainsworth2022git}.
However, efficiently searching for permutation symmetries, that bring all solutions to one basin, is a challenging problem \cite{entezari2022the}. Three main approaches for matching units between two neural networks have been explored. The studies \cite{ainsworth2022git, singh2020model} propose a data-dependent algorithm which associates units across two NNs by matching their activations. Since activation-based matching is data dependent, it helps to adjust permutations to certain desired kinds of classes or domains \cite{singh2020model}. Instead of associating units by their activations, one could align the weights of the model itself \cite{ainsworth2022git, singh2020model}, which is independent of the dataset and therefore the computational cost is much lower. Finally, the third approach is to iteratively adjust the permutation of weights. Many studies \cite{ainsworth2022git, yurochkin2019bayesian, wang2020federated} have proposed to alternate for a number of iterations between finding an alignment and retraining to minimize the loss barriers between SGD minimas. Unfortunately, the proposed approaches so far are either non-differentiable \cite{ainsworth2022git, singh2020model, entezari2022the} or computationally expensive \cite{ainsworth2022git}, making the solution difficult to be extended to other applications, with a different objective. For instance, adapting those methods for domain adaptation by including in the optimization loss the algorithm for weight matching between two models trained on different domains is not trivial.

In this work, inspired by \cite{mena2018learning}, we relax the permutation matrix with the Sinkhorn operator \cite{adams2011ranking} and use it to solve the matching problem in a differentiable fashion. %To reduce the computational cost, previous approaches \cite{ainsworth2022git, singh2020model, wang2020federated} resort to greedy-based algorithms for finding the optimal permutations. 
To avoid the high computational cost for computing gradients in Mena \etal \cite{mena2018learning} proposal, we use the implicit differentiation algorithm proposed by \cite{eisenberger2022unified} which has been shown to be more cost-effective.
%to mitigate such an increase in the computational cost. 
Our re-basin formulation allows defining any differentiable objective as a loss function.

A direct application of re-basin is the merger of diverse models without significantly degrading their performance \cite{garipov2018loss, wang2020federated, ainsworth2022git, benzing2022random, frankle2020linear}. Applications like federate learning \cite{ainsworth2022git}, ensembling\cite{frankle2020linear}, or model initialization \cite{benzing2022random} exploit such a merger by selecting a model in the line connecting the models to be combined. Here to show the effectiveness of our approach, we propose a new continual learning algorithm that combines models trained on different domains. Our continual learning algorithm differs from previous state-of-art approaches \cite{mirzadeh2021linear} because it directly estimates a model at the intersection of previous and new knowledge by exploiting the LMC property observed in SGD-based solutions.


Our main contribution can be summarized as follows:

%\begin{enumerate}
\noindent \textbf{(1)} Solving the re-basin for optimal transportation using implicit Sinkhorn differentiation, enabling better differentiable solutions that can be integrated on any loss. %results on different metrics when compared with the random permutation re-basin.

\noindent \textbf{(2)} A powerful way to use our re-basin method based on the Sinkhorn operator for continual learning, by considering it as a model merging problem and leveraging LMC. %This is possible because our re-basin approach is differentiable and it can be used to easily 

\noindent \textbf{(3)} An extensive set of experiments that validate our method for: (i) finding the optimal permutation to transform a model to another one equivalent; (ii) linear mode connectivity, to linearly connect two models such that their loss is almost identical along the entire connecting line on the weights space; and (iii) continual learning, to learn new domains and tasks while not forgetting the previous ones. %conducted on real-world applications, such as continual and \textcolor{blue}{federated learning}, using various challenging  benchmarks datasets, like Rotated MNIST and Incremental CIFAR-10.
%\end{enumerate}


%Extensive experiments conducted on two challenging public datasets -- YouTube-Objects v1.0 and v2.2 -- that are comprised of unconstrained videos indicate that: (a) standard CAM methods designed for WSOL on still images can achieve a high level of localization accuracy on frames from test set videos; (b) our TCAM method can achieves state-of-art in WSVOL accuracy. Results suggest that TCAM can be adapted for challenging downstream tasks, such as visual object detection and tracking.  

==> Re-basin via Sinkhorn operator/02_related_work.tex <==
\section{Related work}
\label{sec:related}

%%%
\noindent \textbf{Re-Basin.} Recently, in neural network community, re-basin has been demonstrating useful properties. The main goal of such re-basin approaches is to obtain functionally equivalent models in a different region of the weight space following some pre-defined objective. Permutation symmetries are a well-known example of transformations that allows performing re-basin. In particular, Entezari \etal ~\cite{entezari2022the} shows that the invariances of neural networks using random permutations on SGD solutions are likely to have almost zero barriers, and therefore the randomness in terms of permutations does not impact the quality of the final training result of the model. A simulated annealing-based algorithm was proposed for doing a re-basin with an elevated computational cost which makes it impractical to use, especially for bigger models. Ainsworth \etal~\cite{ainsworth2022git} proposed three new re-basin algorithms, that rely on solving linear assignment problems to find permutation matrices that satisfy their encoded objective. The methods shown perform well, especially in achieving linear mode connectivity. On the downside, new objectives are difficult to plug into their framework and their solution uses greedy algorithms which do not guarantee to find the optimal solution, as shown in our experiments. Using a similar approach, Benzing \etal.~\cite{benzing2022random} found strong evidence that two random initialization of a neural network after permutation can lead to a good performance, showing that the random initialization is already in the same loss valley during the initialization. Finally,~\cite{akash2022wasserstein} uses the concepts of Wasserstein Barycenter and Gromov-Wasserstein Barycenter, offering a framework for neural network model fusion with insights about linear mode connectivity of SGD solutions. Even though the previous works presented solutions to perform re-basin by solving linear assignment problems, their approach fails to generalize well for other objectives. Using gradient descent-based algorithms seems to be a more suitable approach.

%%%
\noindent \textbf{Differentiating through permutations.} Permutations are fundamental for diverse applications, especially those that involve aligning and sorting data, and are the core of most current re-basin algorithms. However, the solution space is constrained to the set of binary permutation matrices, which makes differentiation very difficult. Mena \etal \cite{mena2018learning} proposes the Gumbel-Sinkhorn, an extension of the Gumbel-Softmax method, which is a non-differentiable parametrization of a permutation that is approximated by the Sinkhorn operator. Recently, \cite{eisenberger2022unified} proposes a computationally efficient and robust approach to differentiate the Sinkhorn operator. %In~\cite{ainsworth2022git}, different algorithms with permutations are proposed for LMC of SGD solutions in deep learning, making their loss landscape as flat as possible. 
We based our proposal on these studies providing solutions to obtain a differentiable re-basin via permutation. Such an approach simplifies the generalization to other applications such as continual learning and federated learning and makes it easy to integrate into neural networks.

%%%%
\noindent \textbf{Mode connectivity.} Mode connectivity is responsible for demonstrating that the loss minima of different models can be connected in the weight space with almost zero loss barrier, introducing the concept of the basin of equivalent solutions. In their work, Garipov \etal \cite{garipov2018loss} found that the local optima of deep learning models are connected by simple curves. As an application for their proposal, the Fast Geometric Ensembling method was proposed. Almost at the same time, \cite{draxler2018essentially} proposed a Nudged Elastic Band-based method to construct continuous paths between minima of neural networks architectures. Finally, Frankle \etal ~\cite{frankle2020linear} studies the sensitivity of different levels of SGD noise on neural networks. These pioneering works are the basis for applications of mode connectivity, like \cite{ainsworth2022git, mirzadeh2021linear} and ours.

%%%%%
\noindent \textbf{Continual learning.} Continual or incremental learning (CL) has received much attention in the machine/deep learning community, allowing us to adapt models incrementally based on new training data, without forgetting previous knowledge. Catastrophic forgetting~\cite{mccloskey1989catastrophic, ratcliff1990connectionist} occurs when a model that is trained for a task on a new dataset loses information learned to perform well on that task on the original dataset. To address this issue for CL,~\cite{kirkpatrick2017overcoming} proposes Elastic Weight Consolidation (EWC), which smooths the catastrophic forgetting by regularizing neural network parameters with respect to the importance of the weights concerning the previous and actual tasks. Chaudhry \etal ~\cite{chaudhry2019tiny} proposes to use a small number of samples for replay. In their work, the Experience Replay (ER) helps the CL, even with tiny episodic memory, to  improve performance on classification tasks. Closer to our work,~\cite{mirzadeh2021linear} proposes an LMC-based method with replay. Its solution is called Mode Connectivity SGD (MC-SGD), which relies on the assumption that there is always an existing solution that incrementally solves all seen tasks, and they are connected with a linear path consisting of a low value on the loss landscape. Furthermore, MC-SGD utilizes a replay buffer to remember previous tasks for CL. Its efficiency relies on exploring the linear path of low loss to constrain learning, thus performing better than competitors, such as EWC, when less data is presented. However, such an approach has a high computational cost since it requires training independent models for the new task and merging them as a separate step with the model for previous knowledge. Also, the method has been shown to be difficult to reproduce or adapt to new benchmarks \cite{mehta2021empirical}. A compelling scenario for continual learning is the usage of a linear mode connectivity path to keep learning and adapt the model without forgetting the previous knowledge. The trade-off between the flatness of the LMC path and the direction to adapt the loss can be tuned in a way that brings more stability or plasticity depending on the target final solution.










% Backup
%Godfrey et al.~\cite{godfrey2022symmetries} describe groups of symmetries that come from the non-linearity activation of neural networks. 
%Recent works have shown that permutation symmetry can help find neural network models with similar loss landscape properties~\cite{ainsworth2022git, benzing2022random, akash2022wasserstein}. %by using a novel way to study their sensitivity to this noise.}

==> Re-basin via Sinkhorn operator/03_proposed_method.tex <==


\section{Re-basin via the Sinkhorn operator}
\label{sec:proposal}


Let $f_{\theta}(.)$ be a parameterized mapping where $\theta$ represents a vector of parameters within the solution space $\Theta\subset \R^{d}$, where $d$ is the number of parameters in $\theta$. In the deep learning context, $f$ can be seen as a neural network architecture, and $f_{\theta}$ is a model with weights $\theta$. Here, we refer to $\theta$ as a model for simplicity. Consequently, the cost (or error) of a model for a given task can be defined as $\cost(\theta)=\frac{1}{|\sT|}\sum_{(x,y)\in \sT} \loss(f_{\theta}(x),y)$, where $(x,y)\in\sT$ are input and expect output in training set $\sT$, and $\loss$ is an appropriate loss function.

A function $f$ is invariant to a transformation if and only if the obtained transformed function is functionally equivalent to the original mapping. Note that such invariances can also be found between two functions within the family of parametric functions $\{f_\theta\}_{\theta\in\Theta}$. The permutation of neurons is a well-known example of such transformation applied to neural networks that allow obtaining functionally equivalent models, i.e., $f_{\theta_A}(x)=f_{\theta_B}(x), \forall x$. These invariant models are obtained via the permutation transformation or re-basin function, here defined as $\pi\colon \Theta \to \Theta$, which shifts a model to a symmetric region of the loss landscape, $\mathcal{C}(\theta)=\mathcal{C}(\pi_{\mathcal{P}}(\theta))$. In this work $\mathcal{P}=(P_1,...,P_h)$ is a transportation plan with $P_i$ contained in the transportation polytope,
\begin{equation}
  \Pi=\{P\in \R_{+}^{m\times n}|P\indicator_m=\indicator_n,P^T\indicator_n=\indicator_m\},
\end{equation}
\noindent where $\indicator_d=(1,...,1)^{d}$. Without loss of generality, let $f_{\theta}(x)=(\ell_h\circ ... \circ \ell_1)(x)$ be a neural network defined as the composition of $h$ layers such that $\ell_i(z)=\sigma(W_iz+b_i)$. Here, the weights $W_i$ and biases $b_i$ are the parameters of the network,
%$\theta= \{ W_1, b_1, ..., W_h, b_h \}$, 
$\theta= \{ W_i, b_i \}_{i=1}^h$, and $\sigma$ is a non-linear activation function. Then, the re-based model $\pi_\mathcal{P}(\theta)$ can be written as the functionally equivalent mapping:
\begin{equation}
  \ell'_i(z) = \sigma(P_iW_iP^T_{i-1}z+P_ib_i),
  \label{eq:rebasin}
\end{equation}
\noindent where $P_i\in\Pi$ is a valid permutation matrix, and $P_h=P^T_0=\mI$ is the identity matrix.

With regards to permutation invariance, Entezari \etal \cite{entezari2022the} conjectured that re-based SGD solutions are likely to have a low barrier within their linear interpolation $B(\theta_A,\theta_B)\approx 0$, where $B(.)$ is defined as:
\begin{equation*}
  B(\theta_A,\theta_B)=\sup_{\lambda} [[\cost((1-\lambda)\theta_A+\lambda\theta_B)]-
\end{equation*}
\begin{equation}
  [(1-\lambda)\cost(\theta_A)+\lambda\cost(\theta_B)]],
  \label{eq:barrier}
\end{equation}
\noindent and $\lambda\in(0,1)$. This phenomenon is known as LMC \cite{frankle2020linear}, and it is a particular case of the widely studied mode connectivity \cite{garipov2018loss,draxler2018essentially}. Notably, Ainsworth \etal \cite{ainsworth2022git} proposed three approaches that ratify the conjecture in  \cite{entezari2022the} by finding a re-based model $\pi_{\mathcal{P}}(\theta_B)$ with LMC that is near to a target model $\theta_A$. \cref{fig:rebasin} depicts the goal of such re-basin approaches.
%The goal of such re-basin approaches is depicted in \cref{fig:rebasin}. 
%\cref{fig:rebasin-a} shows a portion of the loss landscape for the polynomial approximation task \cite{oswald2020continual} using the method proposed by Li \etal \cite{visualloss}. 
In this figure, we can observe two solutions for the task, $\theta_A$ and $\theta_B$, found through SGD. As shown in \cref{fig:rebasin-b}, the naive path between $\theta_A$ and $\theta_B$ has higher values of the barrier within the line $(1-\lambda)\theta_A+\lambda\theta_B, \lambda\in(0,1)$. On the other hand, and consistently with the results in \cite{entezari2022the,ainsworth2022git}, our re-based model $\pi_\mathcal{P}(\theta_B)$ achieves LMC by successfully finding a transportation plan $\mathcal{P}$ that shift model $\theta_B$ to the same basin of model $\theta_A$.

Although the seminal work by Ainsworth \etal \cite{ainsworth2022git} proposed a highly efficient approach for finding a permutation that minimizes the distances between models, $\argmin_{\mathcal{P}} ||\theta_A - \pi_{\mathcal{P}}(\theta_B)||^2$, their non-differentiable approach provides solutions that are difficult to be extended to other applications with a different objective. Specifically, their algorithms use a formulation based on the linear assignment problem (LAP) to find suitable permutations, meaning any new objective needs to be cast as a LAP which is a hard task in itself.

In this work, a differentiable approach is proposed to perform re-basin that allows defining any differentiable objective as a loss function. Here, we relax the rigid constraint of having a binary permutation matrix $P$, and consequently add an entropy regularizer $h(P)=-\sum P (\log P)$ to the original LAP as proposed by \cite{mena2018learning}. The final equation is then defined as:
\begin{equation}
  S_\tau(X) = \argmax_{P\in\Pi} \langle P,X\rangle_{F}+\tau h(P),
  \label{eq:sinkhorn}
\end{equation}
being $\tau$ a factor that weights the strengths of the entropy regularization term.

The formulation in \cref{eq:sinkhorn} is known as the Sinkhorn operator and can be efficiently approximated by:
\begin{equation*}
  S_{\tau}^{(0)}(X) = \exp\left(\frac{X}{\tau}\right),
\end{equation*}
\begin{equation}
  S_{\tau}^{(t+1)}(X)= \mathcal{T}_c(\mathcal{T}_r(S_{\tau}^{(t)}(X))).
  \label{eq:sinkhorn2}
\end{equation}
where $X\in\R^{m\times n}$ is a soft version of the permutation matrix, $\mathcal{T}_c(X)=X\oslash(\indicator_{m}\indicator_{m}^{T}X)$ and $\mathcal{T}_r(X)=X\oslash(X\indicator_{n}\indicator_{n}^{T})$ are respectively the re-normalization of columns and rows of $X$, and $\oslash$ is the element-wise division. In their work, Mena \etal \cite{mena2018learning} proved that \cref{eq:sinkhorn2} converges to \cref{eq:sinkhorn} when $t\to\infty$. However, in practice, only a finite number of iterations are needed to produce a suitable approximation. 

Although the Sinkhorn operator is reasonably easy to implement within the neural network layers, a significant drawback arises when considering the efficiency of its differentiation. We use the implicit differentiation algorithm proposed by Eisenberger \etal \cite{eisenberger2022unified} to mitigate such an increase in the computational cost. Their method significantly increases the efficiency, and also stability of the training process. The marginals of the generic formulation in \cite{eisenberger2022unified} are defined as $\va=\indicator_m/m$ and $\vb=\indicator_n/n$ to match the re-basin task.

Finally, our proposed Sinkhorn re-basin re-writes the original re-based mapping in \cref{eq:rebasin} as:
\begin{equation}
  \ell'_i(z) = \sigma(S_{\tau}(P_i)W_iS_{\tau}(P^T_{i-1})z+S_{\tau}(P_i)b_i).
  \label{eq:sinkhorn-rebasing}
\end{equation}
where $P_i\in\R^{m\times n}$ is a differentiable cost matrix. In all our experiments, $P_i$ are initialized to the identity matrix. Note that in contrast with  non-differentiable approaches \cite{eisenberger2022unified,ainsworth2022git,benzing2022random}, our method can update all permutation matrices at the same time during optimization.

To show the ability of our proposed Sinkhorn re-basin to minimize any differentiable objective, we provide three examples of cost functions that are minimized without changing the formulation in \cref{eq:sinkhorn-rebasing}. These cost functions are used in the SGD framework to compute the gradient of the weights in our Sinkhorn re-basin network and finally update the permutation matrices to minimize the objective. First, for a data-free objective like Weights Matching \cite{ainsworth2022git}, we directly minimize the squared L2 distance defined as:
\begin{equation}
  \cost_{L2}(\mathcal{P};\theta_A,\theta_B) = ||\theta_A-\pi_{\mathcal{P}}(\theta_B)||^2.
  \label{eq:rebasinl2}
\end{equation}

Given the ability of our method to use differentiable objectives, we introduce two other data-driven cost functions. Inspired by the Straight-Through Estimator in \cite{ainsworth2022git}, we propose a differentiable midpoint cost function to minimize the barrier,
\begin{equation}
  \cost_{Mid}(\mathcal{P};\theta_A,\theta_B) = \cost\left(\frac{\theta_A + \pi_{\mathcal{P}}(\theta_B)}{2}\right).
  \label{eq:mid}
\end{equation}
Since minimizing the midpoint can lead to a multimodal cost path, i.e., lower cost value for $\lambda=0.5$, and higher cost values elsewhere, we propose a cost function that minimizes the cost at random points within the line:
\begin{equation}
  \cost_{Rnd}(\mathcal{P};\theta_A,\theta_B) =\cost\left((1-\lambda)\theta_A + \lambda\pi_{\mathcal{P}}(\theta_B)\right),
  \label{eq:rand}
\end{equation}
with $\lambda$ uniformly sampled at each iteration, $\lambda\sim U(0,1)$.


%%%%%%%%
\section{Re-basin incremental learning}
\label{sec:proposal2}

\begin{figure}[t]
  \centering
  \includegraphics[height=40mm]{images/cl.pdf}
  \put(-80,10){$\theta_i$}
  \put(-32,102){$\pi_{\mathcal{P}_i}(\theta_i)$}
  \put(-130,68){$(\theta_{i}+\pi_{\mathcal{P}_i}(\theta_i))/2$}
  \put(-45,45){$\theta_{i+1}$}
  \put(-34,80){$\delta_{i}$}
  \put(-95,40){\rotatebox[origin=c]{65}{\tiny Low cost region for $\sT_i$}}
  \put(-33,50){\rotatebox[origin=c]{-45}{\tiny Low cost region for $\sT_{i+1}$}}


  \caption{Graphical representation of the intersection of low curvature regions of the loss landscape for task $\sT_i$ (red) and $\sT_{i+1}$ (blue). The goal of our method is to find a re-basin $\pi_{\mathcal{P}_i}(\theta_i)$ that transverses the multitask region using LMC. The final model $\theta_{i+1}$ (\cref{eq:clrebasin_newmodel}) is found in the surroundings of the line by adding a learnable residual $\delta_i$.}
  \label{fig:rebasincl}
\end{figure}

A critical application of re-basin approaches is the ability to merge models without a significant performance reduction. Such a merging is usually done by selecting a model in their connecting line. Applications like federate learning \cite{ainsworth2022git}, ensembling\cite{frankle2020linear}, or model initialization \cite{benzing2022random} have been explored recently for merging models trained on the same task. Here we push the merging based on re-basin further by proposing a new incremental learning approach that fuses models trained on different domains or classes. Our proposed approach relies on a stability-plasticity hyper-parameter that allows us choosing the balance between forgetting and incorporating the new knowledge.

Let $\theta_0$ be an initial model trained over dataset $\sT_0$. Let also $\mathcal{T}=\{\sT_1, \sT_2, ...\}$ be a stream of data where $\sT_i=\{(x_{ij},y_{ij})|x_{ij}\in\sX_i, y_{ij}\in\sY_i\}, 1\leq i\leq N_i$, is a supervised dataset with input $\sX_i$, output $\sY_i$, and $N_i$ data points. Note that the sets $\sT_i$ are also known in continual learning literature as tasks but these are not limited to task incremental learning scenarios, but also include domain and class incremental learning. An incremental or continual learning process seeks to incorporate the new knowledge $\sT_{i+1}$ into the model $\theta_i$ without forgetting how to perform correctly in previous datasets $\sT_0,...,\sT_i$. To this end, 
%Mirzadeh et al. \cite{mirzadeh2021linear} proposed a mode connectivity-based 
the continual learning community has proposed approaches that exploit the fact that multitask low curvature regions usually appear at the intersection of low curvature regions for individual tasks \cite{kirkpatrick2017overcoming,mirzadeh2021linear} (see \cref{fig:rebasincl} for a visual reference). In particular, Mirzadeh \etal \cite{mirzadeh2021linear} approach uses a two steps training where the model $\theta_{i+1}$ is first trained over dataset $\sT_{i+1}$ and then a mode connectivity-based merging finds the model with low loss value on both new and previous knowledge.

In our approach, different from \cite{mirzadeh2021linear}, we directly estimate a model in the intersection of previous and new knowledge by exploiting our differentiable method to obtain the LMC observed in SGD-based solutions. Similarly to the approaches introduced in the last section, our method looks for a re-basin of the given model that minimizes a given objective. For continual learning purposes, a new cost function is introduced such that, similarly to \cref{eq:mid}, the cost of the model in the middle of the line $(1-\lambda)\theta_i+\lambda\pi_{\mathcal{P}_i}(\theta_i),\lambda\in(0,1),$ is minimized for dataset $\sT_{i+1}$, (see \cref{fig:rebasincl}). In such a continual learning scenario, the middle point is the furthest model in the line from high stability points $\theta_i$ and $\pi_{\mathcal{P}_i}(\theta_i)$. %Optimizing the new cost on the middle point allows us to find a model that excels on the new knowledge but fails to retain the previous one, contrary to the extreme of the line. On the other hand, 
Constraining the solution space to the models within the line yields a solution that performs well on the previous task, but does not allow optimal performance on the new task, thus affecting the training plasticity. Similarly to Kirkpatrick \etal \cite{kirkpatrick2017overcoming}, we find well-behaved models for $\sT_{i+1}$ in the neighborhood of our optimization target. This is done by adding a residual vector $\delta_i$ with $l_2$ norm close to zero with a regularization term. Finally, the proposed cost is calculated as:
%to learn jointly a residual model $\delta_i$, which allows for finding better solutions in the surroundings of the line:
\begin{equation}
  \cost_{CL}(\delta_i, \mathcal{P}_i;\theta_i) =  \cost\left(\frac{\theta_i+\pi_{\mathcal{P}_i}(\theta_i)}{2}+\delta_i\right)+\beta||\delta_i||^2.
  \label{eq:clcost}
\end{equation}

During the learning phase, the underlying optimization problem finds:
\begin{equation}
  \delta_i^*, \mathcal{P}_i^* = \argmin_{\delta_i, \mathcal{P}_i} \cost_{CL}(\delta_i, \mathcal{P}_i;\theta_i),
\end{equation}
where $\delta_i^*$ and $\mathcal{P}_i^*$ are found at the same time. Note that the cost in \cref{eq:clcost} can be computed over any knowledge dataset. In this work, a replay method is used by taking the average of \cref{eq:clcost} for current and previous datasets. %Otherwise, optimization in \cref{eq:clcost} should be run for task $\sT_{i+1}$ only. 

A fused model with a balance between previous and new knowledge should be obtained after minimizing the cost in \cref{eq:clcost}. Here, the incremented model at episode $i+1$ is defined as:
\begin{equation}
  \theta_{i+1} =  (1-\alpha)\theta_i + \alpha\pi_{\mathcal{P}_i}(\theta_i)+\delta_i,
  \label{eq:clrebasin_newmodel}
\end{equation}
where $\alpha$ is a hyper-parameter controlling the balance between plasticity and stability. Note that values of $\alpha$ near $0.5$ favors higher plasticity, while values around $0.0$ and $1.0$ give more importance to previous knowledge.






==> Re-basin via Sinkhorn operator/04_results.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=.9\linewidth]{images/figure1.pdf}
    \put(-416,92){$P_0$}
    \put(-365,92){$\hat{P}_0$ from WM}
    \put(-285,92){$\hat{P}_0$ (Ours)}
    \put(-190,92){$P_1$}
    \put(-135,92){$\hat{P}_1$ from WM}
    \put(-56, 92){$\hat{P}_1$ (Ours)}
    \caption{Estimated permutation matrices via  Weight Matching (WM) \cite{ainsworth2022git} and the proposed Sinkhorn re-basin. $P_i$ refers to the expected $10\times 10$ permutation matrix with ones represented in black and zeros in white. The estimated permutations matrix $\hat{P}_i$ shows matching permutations as blue squares and miss-matchings in red and yellow. The permutation matrices $P_i\in\R^{10\times 10}$ correspond with transportation plans of layer $i$, with each layer containing 10 neurons. These matrices correspond with actual permutation matrices from the experiment with random initialization and 2 hidden layers.}
    \label{fig:estimated_permutations}
\end{figure*}

\section{Experimental results and analysis}
\label{sec:results}

The experimental procedure for comparing re-basin approaches follows the same one used by Ainsworth \etal \cite{ainsworth2022git}, while the continual learning experiments follow the standard experimental procedure in incremental learning literature \cite{mirzadeh2021linear}. For all experiments, the mean and standard deviation of results are reported, and were obtained over independent runs with different seeds. We used the original implementation provided by the authors in all cases. We study the effect of re-basin for both classification and regression tasks. Mnist and Cifar10 datasets were used for image classification. The polynomial approximation problems from \cite{oswald2020continual} were used for regression. As backbone architectures, we explored feedforward neural networks with 2 to 8 layers. In all our experiments, we use $t=20$ and $\tau=1.0$ as proposed in \cite{mena2018learning} for the Sinkhorn operator. Furthermore, the corresponding performance measures and hyper-parameters are summarized in each subsection. Additional details on the experimental methodology, e.g., dataset, protocol, and performance measures, are provided in the supplementary material.


%%%
\subsection{Finding the optimal transport}

In this experiment, we measure the ability of both Weights Matching (WM) \cite{ainsworth2022git} and our Sinkhorn re-basin to find the optimal permutation. Similar to our $\cost_{L2}$, the Weights Matching method minimizes the norm between the re-based model and a target model by solving a LAP. The cost function used for our re-basin is the squared L2 distance between models (\cref{eq:rebasinl2}). Note that the objectives are not data-driven, and therefore we only measure the ability of each algorithm to reach the global minima without any context. Each method received a model and a randomly permuted version of it, with the goal of finding the permutation matrices that originated the target re-basin.

For our purposes, 9 datasets are created, each one containing 50 models and a random re-basin, $\sT_i=\{(\theta_{ij},\pi_{\mathcal{P}}(\theta_{ij}))\mid P_k\sim\text{U}(\Pi), \forall P_{k}\in\mathcal{P}\}$, where $1\leq j\leq 50$ is the index of the model within dataset $\sT_i$ and $1\leq k \leq h$ is the number of hidden layers in the neural network. Note that we select random permutation matrices following a uniform distribution, $\text{U}(\Pi)$. Neural networks with two, four, and eight hidden layers were used as base architecture. Additionally, we tested three types of initializations -- random initialization with weights following a normal distribution $\mathcal{N}(0,1)$, hereafter called \emph{Rnd}, and models trained in a third and first-degree polynomial approximation problem, named \emph{Pol3} and \emph{Pol1} respectively. The 9 data set configurations lie within the combination \{Rnd, Pol3, Pol1\}$\times$\{2 hidden, 4 hidden, 8 hidden\}.

\begin{table}[t]
    \centering
    \begin{tabular}{@{}l@{\kern1.0em}l@{\kern1.0em}c@{\kern1.0em}c@{\kern1.0em}c@{}}
        \toprule
        Method                     & Init & 2 hidden $\downarrow$  & 4 hidden $\downarrow$  & 8 hidden  $\downarrow$ \\
        \midrule
        WM \cite{ainsworth2022git} & Rnd  & 6.05$\pm$9.17          & 4.12$\pm$6.58          & 0.50$\pm$1.55          \\
        $\cost_{L2}$ (Ours)        &      & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} \\
        \midrule
        WM \cite{ainsworth2022git} & Pol3 & 0.57$\pm$2.84          & 0.07$\pm$0.46          & 0.01$\pm$0.10          \\
        $\cost_{L2}$ (Ours)        &      & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} \\
        \midrule
        WM \cite{ainsworth2022git} & Pol1 & 0.27$\pm$0.94          & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} \\
        $\cost_{L2}$ (Ours)        &      & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00} \\
        \bottomrule
    \end{tabular}
    \caption{L1 distance between the estimated and expected re-basing with different network initialization and depth. Distances are scaled $\times 10^3$. }
    \label{tab:expot}
\end{table}

\begin{table*}[t]
    \centering
    \begin{tabular}{@{}lllllllll@{}}
        \toprule
                                      & \multicolumn{2}{c}{First degree polynomial} & \multicolumn{2}{c}{Third degree polynomial} & \multicolumn{2}{c}{Mnist}            & \multicolumn{2}{c}{Cifar10}                                                                                                                                                                                  \\
        \multicolumn{1}{@{}l}{Method} & \multicolumn{1}{c}{AUC $\downarrow$}        & \multicolumn{1}{c}{Barrier $\downarrow$}    & \multicolumn{1}{c}{AUC $\downarrow$} & \multicolumn{1}{c}{Barrier $\downarrow$} & \multicolumn{1}{c}{AUC $\downarrow$} & \multicolumn{1}{c}{Barrier $\downarrow$} & \multicolumn{1}{c}{AUC $\downarrow$} & \multicolumn{1}{c}{Barrier $\downarrow$} \\
        \midrule
        Naive                         & 0.31$\pm$0.38                               & 0.62$\pm$0.71                               & 0.25$\pm$0.15                        & 0.58$\pm$0.33                            & 0.34$\pm$0.08                        & 1.07$\pm$0.21                            & 0.73$\pm$0.12                        & 1.23$\pm$0.18                            \\
        WM \cite{ainsworth2022git}    & 0.16$\pm$0.15                               & 0.32$\pm$0.28                               & 0.19$\pm$0.26                        & 0.41$\pm$0.57                            & 0.01$\pm$0.00                        & 0.03$\pm$0.01                            & 0.13$\pm$0.02                        & 0.27$\pm$0.04                            \\
        $\cost_{L2}$ (Ours)           & 0.05$\pm$0.06                               & 0.10$\pm$0.12                               & 0.05$\pm$0.06                        & 0.12$\pm$0.12                            & 0.01$\pm$0.00                        & 0.02$\pm$0.00                            & 0.09$\pm$0.02                        & 0.19$\pm$0.03                            \\
        \midrule
        STE \cite{ainsworth2022git}   & 0.11$\pm$0.10                               & 0.23$\pm$0.22                               & 0.09$\pm$0.07                        & 0.24$\pm$0.23                            & 0.01$\pm$0.00                        & 0.01$\pm$0.01                            & 0.08$\pm$0.01                        & 0.15$\pm$0.02                            \\
        $\cost_{Mid}$ (Ours)          & 0.03$\pm$0.02                               & 0.07$\pm$0.05                               & 0.05$\pm$0.04                        & 0.17$\pm$0.17                            & \textbf{0.00$\pm$0.00}               & \textbf{0.00$\pm$0.00}                   & \textbf{0.02$\pm$0.01}               & \textbf{0.05$\pm$0.01}                   \\
        $\cost_{Rnd}$ (Ours)          & \textbf{0.01$\pm$0.01}                      & \textbf{0.03$\pm$0.02}                      & \textbf{0.01$\pm$0.01}               & \textbf{0.03$\pm$0.03}                   & \textbf{0.00$\pm$0.00}               & 0.01$\pm$0.00                            & \textbf{0.02$\pm$0.01}               & 0.06$\pm$0.01                            \\
        \bottomrule
    \end{tabular}
    \caption{AUC and loss Barrier results of linear mode connectivity for regression datasets (first and third-degree polynomial approximation), and classification datasets (Mnist and Cifar10). The WM method and our Sinkhorn with $\cost_{L2}$ belong to the data-free category, while Straight-Trough Estimator STE, Sinkhorn with $\cost_{Mid}$ and $\cost_{Rnd}$ are data-driven.}
    \label{tab:exp2}
\end{table*}

The Sinkhorn re-basin model was updated using the Adam optimizer with an initial learning rate of $0.1$, and for a maximum of 5 iterations, using early stopping in case of convergence. \cref{tab:expot} summarizes the L1 norm between weights after re-basin, $|\pi_{\hat{\mathcal{P}}}(\theta)-\pi_{\mathcal{P}}(\theta)|$, where $\hat{\mathcal{P}}$ and $\mathcal{P}$ are the estimated and optimal transportation plan, respectively. As expected, our proposal always finds the optimal permutation thanks to its ability to look at all permutation matrices simultaneously. In contrast, the WM results fall short for some scenarios. It is worth mentioning that these results match the ones obtained by Ainsworth \etal in \cite{ainsworth2022git}. In general, the WM algorithm seems to be affected by random initialization, while increasing the network's capacity improves its ability to reach the global minimum. We hypothesize that this is an effect of using a greedy algorithm that optimizes the objective for different layers at each iteration. A deeper inspection of the estimated permutation matrices show that WM reaches local minima close to the expected re-basin, with only a few misplaced permutations (see \cref{fig:estimated_permutations}).

%%%%%
\subsection{Linear mode connectivity}

\begin{figure*}[t]

    \centering
    \includegraphics[width=0.9\linewidth]{images/figure_curves.pdf}
    \put(-31,48){\tiny Naive}
    \put(-31,41){\tiny WM}
    \put(-31,35){\tiny STE}
    \put(-31,28){\tiny $\cost_{L2}$}
    \put(-31,21){\tiny $\cost_{Mid}$}
    \put(-31,14){\tiny $\cost_{Rnd}$}
    \put(-65,-10){\small $\lambda$}
    \put(-220,-10){\small $\lambda$}
    \put(-373,-10){\small $\lambda$}
    \put(-95,102){\small Accuracy Mnist}
    \put(-240,102){\small Loss Mnist}
    \put(-422,102){\small Loss third degree polynomial}
    % \put(-65,109){\small $\lambda$}
    % \put(-220,109){\small $\lambda$}
    % \put(-373,109){\small $\lambda$}
    \put(-95,218){\small Accuracy Cifar10}
    \put(-240,218){\small Loss Cifar10}
    \put(-422,218){\small Loss first degree polynomial}
    \caption{Example of linear mode connectivity achieved by Weight Matching (WM) \cite{ainsworth2022git}, Straight-Through Estimator (STE) \cite{ainsworth2022git}, and our Sinkhorn re-basin with $\cost_{L2}$, $\cost_{Mid}$, and $\cost_{Rnd}$ costs for a neural network with two hidden layers. Accuracy and loss are shown for the Mnist and Cifar10 classification, while only the L2 loss is shown for the regression tasks. For Mnist, we include an amplified version of the loss and accuracy for better comparison.}
    \label{fig:LMC}
\end{figure*}

To verify the conjecture of Entezari \etal \cite{entezari2022the}, we measure the ability of our method to find linear connectivity between SGD modes after re-basin one of them. For this experiment, four datasets are employed -- first and third-degree polynomial regression tasks \cite{oswald2020continual}, along with the classical classification benchmarks, Mnist and Cifar10. Our experiment follows a similar setup to the one described by \cite{ainsworth2022git}, i.e., two networks were trained over the same dataset, and we performed the re-basin of one of them, hoping to reach the same basin as the unchanged model. The experiment was repeated 50 times for every dataset, and each method saw the same two networks. To measure the ability of the different approaches to find LMC, we use the Barrier \cite{frankle2020linear} (\cref{eq:barrier}) and Area Under the Curve (AUC) over the estimated cost curve within the linear path.
%\begin{eqnarray}
%    AUC = \int_{\lambda=0}^{1}\cost((1-\lambda)\theta_A+\lambda\theta_B)\text{d}\lambda.
%\end{eqnarray}
With both measures, the best performance is achieved when a method provides a low value, with a lower bound of 0.
%Note that the lower the value, the best performed is the method with both metrics having a lower bound of 0. 

We compare our approach with different objectives -- L2 (\cref{eq:rebasinl2}), Middle point (\cref{eq:mid}), and Random lambda (\cref{eq:rand}) with the recently introduced Weights Matching (WM) and Straight-Through Estimator (STE) \cite{ainsworth2022git}. \cref{tab:exp2} reports the performance of the methods for each dataset. All experiments used a neural network with two hidden layers. As seen in the table, our methods outperform state-of-art methods with (first three rows) and without considering the data (last three rows) during re-basin. Specifically, our $\cost_{L2}$ method exceeded WM for both AUC and Barrier measures for all datasets, except Mnist where no significant differences were observed. In the data-driven category, our other proposals outperform the state-of-art STE approach for AUC and Barrier. In particular, our $\cost_{Rnd}$ loss showed the best results, comparable to our $\cost_{Mid}$ for more challenging scenarios like Cifar10. As a general point, all methods provide a significant improvement over the naive path.

%Note that our method is not limited to neural networks (e.g., MLPs and DNNs), but can also perform guided re-basin for convolutional networks like in \cite{ainsworth2022git}. 
We show the obtained loss and accuracy curves over the linear path before doing a re-basin (naive) and after applying WM, STE, and Sinkhorn with $\cost_{L2}$, $\cost_{Mid}$, and $\cost_{Rnd}$ methods in \cref{fig:LMC}. An interesting observation is that $\cost_{Mid}$ tends to find multi-modal cost curves with a valley at $\lambda=0.5$, similarly to STE.




%%%
\subsection{Incremental learning application}

\begin{table*}[h!]
    \centering
    \begin{tabular}{@{}lllllll@{}}
        \toprule
                                             & \multicolumn{2}{c}{Rotated Mnist}       & \multicolumn{2}{c}{Split Cifar100}                                                                                                  \\
        \multicolumn{1}{@{}l}{Method}        & \multicolumn{1}{c}{Accuracy $\uparrow$} & \multicolumn{1}{c}{Forgetting $\downarrow$} & \multicolumn{1}{c}{Accuracy $\uparrow$} & \multicolumn{1}{c}{Forgetting $\downarrow$} \\
        \midrule
        Finetune                             & 46.28$\pm$1.01                          & 0.52$\pm$0.01                               & 35.41$\pm$0.95                          & 0.49$\pm$0.01                               \\
        EWC~\cite{kirkpatrick2017overcoming} & 59.92$\pm$1.71                          & 0.34$\pm$0.02                               & 50.50$\pm$1.33                          & 0.24$\pm$0.02                               \\
        LwF~\cite{li2017learning}            & 61.86$\pm$3.66                          & 0.29$\pm$0.06                               & 41.43$\pm$4.06                          & 0.51$\pm$0.01                               \\
        %Rebasin /wo replay (Ours)            & 53.17$\pm$1.40                     & 0.40$\pm$0.02                      & 38.44$\pm$1.25                     & 0.35$\pm$0.03                      \\
        %\midrule
        A-GEM~\cite{chaudhry2018efficient}   & 68.47$\pm$0.90                          & 0.28$\pm$0.01                               & 44.42$\pm$1.46                          & 0.36$\pm$0.01                               \\
        Rebasin /w replay (Ours)             & \textbf{78.14$\pm$0.50}                 & \textbf{0.12$\pm$0.01}                      & \textbf{51.34$\pm$0.74}                 & \textbf{0.07$\pm$0.02}                      \\
        \midrule
        Joint training                       & 90.84$\pm$4.30                          & 0.00                                        & 60.48$\pm$0.54                          & 0.00                                        \\
        \bottomrule
    \end{tabular}
    \caption{Performance of our proposed and state-of-art methods on the continual learning benchmark datasets over 20 episodes.}
    \label{tab:cl}
\end{table*}

Although several authors have proposed methods to combine models trained over subsets of some domain, e.g., federate learning \cite{ainsworth2022git}, ensembling \cite{frankle2020linear}, and model initializations \cite{benzing2022random}, this paper explores the idea of obtaining a model that can learn a new knowledge without forgetting the previous one. To this end, this experiment seeks to compare our method with other well-known and state-of-art continual learning approaches from the literature. Since our proposal can fit the regularization techniques that use replay, we compare it with different algorithms within this category. In particular, we compared with 3 regularization-based approaches -- elastic weight consolidation (EWC) \cite{kirkpatrick2017overcoming}, learning without forgetting (LwF) \cite{li2017learning}, and average gradient episodic memory (A-GEM) \cite{chaudhry2018efficient}. The average accuracy
%\begin{equation}
%    \text{Acc}_{E,j}=\frac{1}{E}\sum_{j=1}^{E} \text{accuracy}(\theta_{i},\sT_{j})
%\end{equation}
was calculated to measure the overall performance of model $\theta_i$ in the first $E$ episodes $\sT_{j}$. In addition, the forgetting measure
%\begin{equation}
%    \text{F}_{E,j}=\displaystyle\frac{1}{E-1}\sum_{j=1}^{E-1}\max_{i} (\text{Acc}_{i,j}-\text{Acc}_{E,j}),
%\end{equation}
averages the forgetting in terms of accuracy for each domain or task in episode $E$.
%As observed in this last equation, lower values of forgetting are better.

Given the variety of libraries and implementations, we limited our comparison to reproducible models that could be used in the Avalanche environment \cite{lomonaco2021avalanche}. All measures, benchmarks, networks, and algorithms, including our own, were implemented using this framework. While we attempted to  incorporate other recent approaches like MC-SGD\cite{mirzadeh2021linear} and Stable SGD \cite{mirzadeh2020understanding} into Avalanche, a high discrepancy was observed w.r.t. their reported results and, therefore, we restrain ourselves from including them in our study. Difficulties in adapting MC-SGD to new conditions has also been observed by other authors \cite{mehta2021empirical}.

We focused our experiments on low episodic memory scenarios, using only five examples per class for both benchmarks in methods that rely on memory replay (A-GEM and our method). Similar to \cite{mirzadeh2021linear}, we used a neural network with two hidden layers and 256 neurons for the Rotated Mnist benchmark. For the Split Cifar100 benchmark, a multi-head resnet18 was used following the settings in \cite{mirzadeh2021linear,mirzadeh2020understanding}. Since our current Sinkhorn re-basin network implementation does not support residual connections, we only apply the re-basin to linear layers.

\cref{tab:cl} shows the accuracy and forgetting performance of methods on the benchmarks Rotated Mnist and Split Cifar-100 datasets using 20 episodes. Our method outperforms the others, and still achieves better or comparable performance than those reported in \cite{mirzadeh2020understanding}. The reader should pay special attention to the low values of forgetting achieved using our re-basin approach. This is a consequence of setting the value of  $\alpha=0.8$ when fusing the models (\cref{eq:clrebasin_newmodel}). A-GEM is ranked second in accuracy and forgetting for Rotated Mnist. LwF showed a similar forgetting to A-GEM in this benchmark. On Split Cifar100, EWC ranked second for both measures. Despite having similar accuracy to our approach, the high forgetting value suggests stability issues.



==> Re-basin via Sinkhorn operator/05_conclusion.tex <==
\section{Conclusion}
\label{sec:concl}

In this work, a new method based on the implicit Sinkhorn operator is proposed that estimates a permutation matrix which makes two neural network models equivalent. With respect to previous work, such as weight matching, our method is: (i) more flexible, because it is differentiable and can be applied with any loss, (ii) estimates the permutations for all layers at the same time, avoiding getting stuck in local minima, (iii) more accurate, as shown in our experimental evaluation on well-known benchmarks. First, our experiments yield perfect results when our approach was evaluated to produce the optimal permutation between a model and its artificially permuted transformation.  We have also used our approach for linear mode connectivity, showing better connectivity (lower loss barrier) than weight matching.  Finally, we showed that our efficient and differentiable approach for re-basin can easily be applied to the challenging task of continual learning, producing results that are comparable to, or better than state-of-art approaches. As a limitation to our work, we observed from our experiments and analysis of the literature that linear assignment problems solved with greedy Hungarian-based approaches are generally more efficient in terms of memory than the Sinkhorn operator.


==> Re-basin via Sinkhorn operator/06_limitations.tex <==
%\section{Limitations}
%\label{sec:lim}

%From our experiments and analysis of the literature, linear assignment problems solved with greedy Hungarian-based approaches are generally faster and more efficient in terms of memory than the Sinkhorn operator. Additionally, for the moment, our Sinkhorn re-basin network only supports multi-layer perceptrons and basic convolutional neural networks without skip/residual connections.

==> Re-basin via Sinkhorn operator/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

